Many Perception Tasks are Highly Redundant Functions of their Input Data

We show that many perception tasks, from visual recognition, semantic segmentation, optical flow, depth estimation to vocalization discrimination, are highly redundant functions of their input data. Images or spectrograms, projected into different subspaces, formed by orthogonal bases in pixel, Fourier or wavelet domains, can be used to solve these tasks remarkably well regardless of whether it is the top subspace where data varies the most, some intermediate subspace with moderate variability--or the bottom subspace where data varies the least. This phenomenon occurs because different subspaces have a large degree of redundant information relevant to the task.

==> notation.tex <==
\glsdisablehyper
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{dft}{DFT}{Discrete Fourier Transform}
\newacronym{aee}{AEE}{Avergage Endpoint Error}

==> sections/checklist.tex <==
% !TEX root = ../neurips.tex

\clearpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit.

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA).
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize}
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide empirical evidence for the main claims made in the paper across multiple problems in perception spanning classification, depth estimation, semantic segmentation and optical flow prediction which are diverse and complex tasks (in \cref{s:results}). Additionally, we have an extensive appendix with provides additional evidence regarding the main claims made in the paper.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
    %     \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers.
    %     \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
    %     \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    % \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \cref{s:limitations} is dedicated to discussing the limitations of our results. We also clearly articular assumptions made in our work, either using footnotes and in~\cref{s:discussion}.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper.
    %     \item The authors are encouraged to create a separate "Limitations" section in their paper.
    %     \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
    %     \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
    %     \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
    %     \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
    %     \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
    %     \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    % \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The results developed in this work are empirical.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include theoretical results.
    %     \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
    %     \item All assumptions should be clearly stated or referenced in the statement of any theorems.
    %     \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
    %     \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
    %     \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    % \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper j(regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Experimental details are discussed in~\cref{s:setup}. All code that was used to create the experiments has been provided as a part of the supplementary material, and will be made public after the review process.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
    %     \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable.
    %     \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
    %     \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
    %     \begin{enumerate}
    %         \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
    %         \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
    %         \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
    %         \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
    %     \end{enumerate}
    % \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All code that was used to create the experiments has been provided as a part of the supplementary material, and will be made public after the review process.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that paper does not include experiments requiring code.
    %     \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
    %     \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
    %     \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
    %     \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
    %     \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    % \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In \cref{ss:network}, we provide details regarding the optimizer, learning rate schedule and the specific details of the architecture. We have also provided extensive details in~\cref{s:results} to understand and reproduce these results.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
    %     \item The full details can be provided either with the code, in appendix, or as supplemental material.
    % \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We did not calculate error bars in our experiments. Our experiments are computationally intensive and required over 1000 GPU hours. We provide results on CIFAR-10, ImageNet, Cityscapes, ADE20K and M3ED or different perception tasks with dense predictions. Each point in our figures refers to a deep network trained on different data, e.g., different band pass, high pass and low pass filters, in different bases (PCA, Fourier and wavelets). We could have, in principle, calculated error bars for these points using bootstrap. But that would be prohibitively expensive.
    Importantly, at no point in the paper we compare the curves against each other or identify small trends in them to make claims. The claims in this paper are very clear, e.g., ``a model trained on Imagnet using images projected in the Fourier frequency band of indices 30-45 gets 65\% accuracy''. Our point is simply that this accuracy is extremely large, compared to say, the chance accuracy of 0.1\% on Imagenet.
    Having error bars on 65\% would not make this claim any more reliable.
    Altogether, our evidence is substantial: across different modalities, neural architectures, datasets, multiple basis, and different evaluation metrics. This evidence is also strongly corroborated by totally independent concepts such as the partial information decomposition and Shapley values.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
    %     \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
    %     \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
    %     \item The assumptions made should be given (e.g., Normally distributed errors).
    %     \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
    %     \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
    %     \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
    %     \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    % \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In addition to the experimental results that are discussed here, there a substantial number of secondary experiments, failed attempts, that are not reported. The experiments in this paper required approximately 1000 GPU hours. We used a combination of AWS EC2 instances with Nvidia A30 GPUs and a cluster with an assortment of GPUs(RTX 4090, L40, A40).
    %\todo{Rahul: estimate the number of GPU hours for the experiments in the entire paper}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
    %     \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
    %     \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
    % \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We did not use human subjects or participants in these experiments. All our datasets are public ones that are used very commonly in the published literature. We do not anticipate societally harmful consequences of this research.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
    %     \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
    %     \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    % \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is foundational work and it is not tied to any particular application or deployment. We do not anticipate negative social impact. 
    %Down the line, when this line of research matures and it is deployed for making predictions on users, we anticipate a lot of positive social impacts, e.g., prospective learning may enable us to deploy ML models without having to retrain them as data changes over time. This improves performance because it prevents the predictions from deteriorating, but it also leads to other benefits in terms of economic and computational resources necessary to serve ML models.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that there is no societal impact of the work performed.
    %     \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
    %     \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
    %     \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
    %     \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
    %     \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    % \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only use existing public datasets, all appropriately cited in the paper.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper poses no such risks.
    %     \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
    %     \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
    %     \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    % \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only use existing public datasets (appropriately cited in the paper). No new assets are created from this paper.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not use existing assets.
    %     \item The authors should cite the original paper that produced the code package or dataset.
    %     \item The authors should state which version of the asset is used and, if possible, include a URL.
    %     \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
    %     \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
    %     \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
    %     \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
    %     \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    % \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No assets are created in this paper.
    \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not release new assets.
    %     \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
    %     \item The paper should discuss whether and how consent was obtained from people whose asset is used.
    %     \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    % \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing experiments or research with human subjects.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
    %     \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
    % \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing experiments or research with human subjects.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
    %     \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
    %     \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    % \end{itemize}

\end{enumerate}


==> sections/old_results.tex <==
% !TEX root = ../neurips.tex

\section{Results}
\label{s:results}

We elaborate upon the experimental setup in~\cref{s:setup}.

\subsection{Both input data and the task is effectively low-dimensional, very few dimensions capture most of the variance}
\label{s:result_sloppy}

\cref{fig:fig1} shows that Sloppy spectra contain a small number of large eigenvalues and a long tail of small eigenvalues which means that few dimensions capture most of the explained variance. For example in CIFAR10, the first 5 eigenvalues capture 90.11\% of the explained variance and the remaining 3067 dimensions capture a mere 9.89\% of the explained variance. The spectra of the outputs of perception tasks (segmentation, optical flow and depth prediction) are also sloppy (\cref{fig:slopp_spectra}). Both the inputs and outputs of typical tasks are effectively low-dimensional objects.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{imgs/task_sig_vals.pdf}
    \caption{\textbf{The Eigenspectrum is sloppy for all tasks.} Singular Value Spectrum of natural image inputs and output tasks (depth, semantic segmentation, and optical flow)  are sloppy. We find that earlier singular values correspond to low-frequency basis elements and later singular values correspond to high-frequency basis elements.}
    \todo[inline]{RR: larger linewidth, much larger font size. use figsize = (10,10) or so. minor and major grid on the background. is it singular value or the eigenvalue that you are plotting? x-axis should be ``Index of sorted eigenvalue'', y-axis is ``Eigenvalue''. Legend should be ``Depth estimation''. Change `Image' to `Classification'. remove the title. output spectrum.}
    \label{fig:slopp_spectra}
\end{figure}
% An important aspect to both the input data distribution and output data distribution  is both display a sloppy spectrum, showcasing very few large magnitude eigenvalues and a long tail of small magnitude eigenvalues. This showcases these set of perception tasks are not complicated high-dimensional functions, but live in a low-dimensional space, we conjecture helps with learning. Another interesting point of looking at each of the spectra is that original input distribution has the largest of the spectrum, while all task lie below it. This points to tasks are a different manifestation of the input distribution that are lower-dimensional than the input. Take for example the task of optical flow, rather than needing to represent all possible combinations of patches moving to the right, we instead have a single right moving flow value for each of these tasks in the output space. Hence, the tasks are essentially simpler than the input distribution. 

\begin{wrapfigure}{r}{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/mi_all.pdf}
    \caption{\textbf{Images projected onto most eigenspaces have non-zero mutual information with the label.}
        We plot the mutual information between the projection of images onto eigenspaces with 10 contiguous eigenvectors and the labels, using 3 different mutual information estimators. While the top few eigenspaces have the highest mutual information with the labels, the tail also has information relevant to the labels. }
    \label{fig:mi_labels}
    \todo[inline]{RR/AB: x-axis should be ``Index (i) of sorted eigenvalue'', y-axis is ``I(P\_iX, Y) (nats)''. Explain in the caption that $P_i$ is the projection matrix onto the $i^{\text{th}}$ eigenvector.}
\end{wrapfigure}

In line with this belief, the traditional wisdom in machine learning is to project the data onto the top few eigenvectors of PCA in order to solve a downstream task; this choice is rooted in principle of parsimony since the top few eigenvectors capture the largest explained variance for a fixed number of dimensions. This also motivates reconstruction as an objective for self-supervised learning; linear auto-encoders recover the solution of PCA~\citep{baldi1989neural}.


To understand the importance of different eigenvectors, we measure the mutual information between the projections of images onto different eigenspaces in~\cref{fig:mi_labels}; each eigenspace consists of 10 contiguous eigenvectors. We find that projections onto eigenspaces containing the larger eigenvectors have higher mutual information with the labels which we expect. However, there is another surprising observation---the tail also has non-zero mutual information with the labels. Does the tail have information relevant to perception tasks or is this information redundant?


\subsection{Many subspaces of the input data are useful for perception tasks}
\label{s:result_redundancy}

To understand which subspaces are important, we project the images onto Eigen, Fourier and wavelet decompositions of the inputs and train deep networks using the projected images. We consider high-pass, loss-pass and band-filters which consider projectsions onto Eigenvalues (or frequencies) which are bigger, smaller or a band of Eigenvalues (or frequencies). We conduct this experiment across of range of perception tasks (flow, depth segmentation, classification) and an array of datasets (CIFAR10, ImageNet, M3ED, Chairs, Cityscapes). \textbf{We find the entire spectrum achieves low classification or mean-squared error on most if not all tasks when trained using supervised learning} (\Cref{fig:imagenet,fig:perception_err}). Note that this redundancy is very different~\citet{attneave1954some,barlow1989unsupervised,barlow2001redundancy} which is primarily about redundancy in pixel space and is related to the sloppy nature of input spectra. Our results point to redundancy with respect to typical tasks and suggests that even the tail of the spectra (which we usually discard when building efficient codes) can be used to tackle the task. We find that there is more information in the head than the tail and there are diminishing returns from adding new eigenvectors or frequencies.


\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{imgs/imagenet/imagenet_panel1.pdf}
    \caption{\textbf{Almost all eigenspaces, radial frequency bands and wavelet coefficients are useful for classification and contain redundant information for classification tasks like CIFAR10 and ImageNet}. We plot the test accuracy (for CIFAR10 (top) and ImageNet(bottom) of models trained on images projected to different subspaces. For ImageNet, all frequency bands  achieve accuracy bands achieve an accuracy greaterthan 60\%. We see similar trends for CIFAR10 (top) too. This points to redundant information being present across the entire spectrum for classification, even if the classes are not easily recognizable to the human eye when projected to higher frequencies (left). Furthermore, the head of the spectrum usually contains more information than the tail.}
    \label{fig:imagenet}
    \todo[inline]{RR/AB: fill in the white space in this panel. make everything much bigger. not clear what $\FF$ is referring to. y-axis of plots should not have (\%); this way it will also not overlap with the 1.0. change the title to ``CIFAR-10'' and ``Imagenet'' respectively. remove the legend for all the figures except one.}
\end{figure}

% shapley values
% the same story is true for features
% you do not need the tail to predict well. so we should not be worried that fitting to the tail is slow.
% show the calculation with Saxe's linear model for the convergence rate of reconstruction.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{imgs/acc_table}
    \caption{\small \textbf{Across multiple perception tasks, pass band filters have a consistently low error rate or mean average error}. A) Validation Depth Error Spectrum Experiments for U-Net architecture, B) Validation Semantic Segmentation Error Spectrum Experiments for U-Net architecture, C) Validation Depth Error Spectrum Experiments for Efficient Transformer architecture, D) Validation Semantic Segmentation Error Spectrum Experiments for Efficient Transformer architecture, E/G) Validation \gls{aee} Optical Flow Spectrum Experiments for U-Net architecture, F) Validation \gls{aee} Optical Flow Spectrum Experiments for Efficient Transformer architecture }
    \label{fig:perception_err}
    \todo[inline]{RR/AB: use the exact same template as the other figures (colors, font sizes etc). make each figure as a separate PDF; makes it easier to move around figures. use plt.savefig(..., bbox\_inches='tight') if you are not doing it already to save whitespace around the figures. no need to have U-Net in the title. on y-axis ``Error'' instead of ``Error rate''. change y-axis to ``MAE'' instead of repeating ``Depth MAE''. better still, you can say the full thing: ``Mean absolute error'', and ``Average endpoint error''. be consistent: the F in ``Center frequency'' is capitalized here and it is not in the figure above. plots should not have more than 5-6 ticks on the y or x axis. use xlim and ylim for each figure that are ``round numbers''. legend should be similar as well `Low pass', `High pass' and `Pass band'. remove the legend for all the figures except one.}
\end{figure}


To measure the contribution of each subspace to the task, we approximate the Shapley values of different bands in~\cref{fig:shapley,fig:shapley_cifar}. The Shapley values are used in co-operative games, to find contribution of each individual to the co-operative task. In our case, we use Shapley values to find the contrbution of each band to the classification task; the sum of the Shapley values is equal to the classification error when we use the entire image. The Shapley values show that the head of the spectrum is important for classification, segmentations and depth prediction, however predicting the flow requires the some of the higher frequencies and is an exception to this general trend.

% \begin{remark}[Why are masked auto-encoders slow to converge?]
% \label{rem:mae}
% % you do not need the tail to predict well. so we should not be worried that fitting to the tail is slow.
% \end{remark}
\todo{Rahul: AE calculations for optimization process}

% \begin{remark}
% showed the result that choosing a certain \% of the variance of the tail eigenvalues always leads to better performance across classification tasks. In this study, we further inspect this claim across a variety of new tasks, including semantic segmentation, optical flow, and depth prediction. In this study, we performed a similar analysis to \citet{randall_recon}, except we inspected each of our tasks over a variety of different regions of the spectra.
% \end{remark}


\begin{remark}[\textbf{Contrary to~\citet{balestriero2024learning}, our results suggest that any part of the spectrum can be used effectively for perception tasks}]
\label{rem:lecun}
% you do not need the tail to predict well. so we should not be worried that fitting to the tail is slow.
% \citet{baldi1989neural}, show that reconstruction using linear networks recovers the top-k principal components.
\citet{randall_recon} argue that the the tail of the spectrum is important for classification, however our results suggest that the head of the spectrum suffices for classification. \citet{randall_recon} hypothesize masked auto-encoders are slow to train due to the difficulty in fitting the tail, which they argue is critical for classification.
However~\cref{fig:shapley_cifar} points to how the first 500 eigenvectors are more important than the last 500 eigenvectors. This throws into question why masked auto-encoders are sub-optimal for classification and rules out the hypothesis that it is due to the inability to capture the tail. We note that the two results are not at odds since \citet{balestriero2024learning} define the head with respect to explained variance, which includes very few eigenvectors.
\end{remark}


\begin{remark}[Noise in the tail]
\label{rem:noise_tail}
\end{remark}
\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{Neurips24/imgs/noise_spec.png}
    \label{fig:image_noise}
    \caption{Image Noise Exps}
\end{figure}


From the above, we found that the samples in the tail of the eigenspectrum exists instability over dataset bootstraps. We wanted to further understand should this be due to random sampling effects or noise present in the tail. Therefore, we looked at image noise estimation techniques for additive white Gaussian noise in the image spectrum. Image noise estimation techniques exists in two flavors: 1) Estimate noise based on the spectral statistic and assume the tail is the noise~\cite{PCA_Noise_Est,Image_Noise_Spec}, 2) Estimate noise based on image regions, such as flat nearly homogeneous patches~\cite{ivhc_noise}. As we want to inspect the noise in the tail, we use the estimator by \citet{ivhc_noise}, that estimate the image noise level by finding homogeneous patches in the image frame and estimating the image variance on these patches. We found for our image set of M3ED the variance to be: $\sigma=1.19$. In Fig. \ref{fig:image_noise}, we showcase the original spectrum along with the noise spectrum in natural images. Overall, the noise spectrum is constant over eigenvalues, and showcases a larger signal to noise ratio in the head than the tail. The image noise is not higher magnitude than the entire spectrum, and shows signal is stronger than the noise even in the tail. 


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.32\linewidth]{imgs/shapley/svd_v2.pdf}
    \includegraphics[width=0.32\linewidth]{imgs/shapley/fft_v2.pdf}
    \includegraphics[width=0.32\linewidth]{imgs/shapley/wave_v2.pdf}
\caption{\textbf{The Shapley values suggest that the head of the spectrum is most important for classification on CIFAR-10.} To explain which components are most important towards accuracy ,we approximate Shapley values by solving an optimization problem (\cref{ss:shapley}) Most of the tail is helpful for classification, and contains information for the classification task.}
    \label{fig:shapley_cifar}
    \todo[inline]{RR/AB: x-axis: let's say ``Eigenvalue (passband)''? y-axis can be just SHAP value, no need for approximate (all of them are approximate...). same ylim for all three figures; you can even remove the y-axis for two of the figures, saves space. draw a horizontal line at y=0, this way the bars will stand out upon it.}
\end{figure}


\subsubsection{Differences between the tasks}

% \paragraph{Classification}

\paragraph{Optical Flow}
For optical flow with both the E-Former and U-Net, the validation \gls{aee} decreases with increased cut-off frequency until a threshold where a negligible decrease in \gls{aee} is seen. As for the high pass filter, we find that decreasing the cut-off frequency, thereby increasing the number of frequencies present, always leads to a decrease in error. Next, across our pass band experiments, we find that using a lower center frequency consistency led to better \gls{aee}. These results lead to the conclusion that more relevant information for optical flow is maintained in the head of the spectrum as opposed to the tail. We also performed all of these experiments for phase-based filters that set that instead of masking the amplitude spectrum, mask the phase spectrum. Across the board for low pass, high pass, and bandpass experiments, we find similar patterns. Next, we inspected the $\text{sinc}(kx)=\sin(kx)/(kx)$ over various frequencies and found increasing the frequency or removing more spatially separated information still yields good performance. This points to the idea that nearby blocks of frequency information contain redundant information that can be recovered from one another. In a set of random passband filters, we find no clear pattern as to the set chosen and performance.

\paragraph{Semantic Segmentation}
The first observation we make for semantic segmentation is similar to optical flow in both the E-Former and U-Net the validation segmentation error decreases with increased cut-off frequency until a threshold where a negligible decrease in depth error is seen. However, we note that this decrease in error is much less than in optical flow. For high pass, we find a similar factor that increasing the high pass cut-off frequency decreases the error but more subtly. As for the pass band experiments, we find no clear pattern in the UNet, although in the efficient former we find that low frequencies lead to lower segmentation error. In a set of random pass band filters, we find no clear pattern as to the set chosen and performance.

\paragraph{Depth}
The first observation we make for depth prediction is similar to optical flow in both the E-Former and U-Net the validation depth error decreases with increased cut-off frequency until a threshold where a negligible decrease in depth error is seen. Again similar to optical flow for the high pass with the efficient transformer we find that decreasing the cut-off frequency, thereby increasing the number of frequencies present, always leads to a decrease in error. However, in the U-Net architecture, this effect is less pronounced than in the efficient transformer. Finally for the pass band, in both cases, it appears that there is no correlation between the center frequency and depth error. At least in the case of the Efficient Transformer, these results point to the head containing more relevant information than the tail for depth prediction.  In a set of random pass band filters, we find no clear pattern as to the set chosen and performance.


\subsection{Understanding redundant information using partial information decomposition}
% \subsection{All bands have lots of redundant information about the task, some synergistic information, but very little unique information}
% this may be a crude approximation, but it is corroborated by Result 1.

While both the head and the tail have information pertinent to the classification task, we do not know if the information and tail provides information that is redundant or complementary. To this end, we make use of the partial information decomposition (PID) of the mutual information $I(X_1, X_2, ; Y)$. Given variables $X_1$ and $X_2$, the PID decomposes the mutual information into redundant ($R$), synergistic ($S$) and unique information ($U_1$, $U_2$). However, the PID is notoriously hard to calculate since we do not know $P(X_1, X_2, Y)$. We hence make the rather crude approximation that $X_1$ and $X_2$ and $Y$ are jointly Gaussian, which allows us to compute the PID easily. Under this assumption, we compute the PID for CIFAR-10 (in~\cref{fig:pid_cifar}) We find that pair of subspaces have a high amount of redundant and unique information but small amounts unique information.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/pid/mi_svd.pdf}
    \caption{\textbf{Partial information decomposition of CIFAR10 suggests that different bands have high amounts of redundant and synergistic information.} The values in the plot are the logarithm of information and values in cell $(i, j)$ corresponds to the PID for subspaces $i$ and $j$. The unique information in each component is multiple orders of magnitude smaller than the synergistic information. Furthermore, the unique information reduces as we move into the tail of the spectrum. However, we note that these results assume the inputs and labels to be jointly Gaussian, which could be a poor approximation. For decomposition plots for frequencies and wavelets see~\cref{fig:pid_cifar_v2}}
    \todo[inline]{RR/AB: x-axis: let's say ``Eigenvalue (passband)''? make separate PDF for each matrix. we might want to make synergistic and unique small... Title should be ``Redundant information (nats)'', ``Synergistic information (nats)'' etc. do you think we can use viridis to make it look better? i would even just use single hue like gray; since numbers are in the boxes, we can remove the colorbar. see Fig S.2 in https://arxiv.org/abs/2308.03175}
    \label{fig:pid_cifar}
\end{figure}


\subsection{If there is information in every subspace, which subspace does a deep network use?}

Given that different subspaces have different amounts of redundant, synergistic and unique information, does a network trained on the original image optimally exploit this information? Does it make use of the synergistic information across the different bands and extract the unique information relevant to the task from the head of the spectrum? To study this, we consider a networks trained on original images (of CIFAR10 and ImageNet-1k) but evaluate trained models on images projected onto different subs-spaces. If the accuracy drops significantly after projecting the image onto a particular subspace, we take this observation as evidence that the trained networks likely uses information present in that subspace. In~\cref{fig:ablation_classification,model_sens}, we find that most models only leverage the the head of the spectrum and there is synergistic information and unique information in the tail that is unused. 
% The results also suggest that adversarial attacks must modify the head of the spectrum in order to change the predictions made by the model, since applying a low-pas filter on the inputs seemingly results in no changes to the classification accuracy.

\begin{figure}[htb]
    \centering
    \includegraphics[width=5.5in]{Neurips24/imgs/rein.pdf}
    \caption{Through our above analysis, we showed how models can use different subsets of frequency bands to yield accurate task performance. This figure shows the sensitivity of trained models with all the features to different frequency bands. Overall you can see an interesting phenomenon in the pass band filters all showing a low-frequency bias, known in the ML community as Spectral Bias.
  }
    \label{fig:model_sens}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.425\linewidth]{imgs/cifar10_abl_svd.pdf}
    \includegraphics[width=0.45\linewidth]{Neurips24/imgs/imagenet/imagenet_abl_fft.pdf}
    \caption{\textbf{Trained networks exhibit a strong bias to use information present in the head of the spectrum and largely ignore the tail}. The ImageNet accuracy drops to 0.1\% if we exclude the radial frequencies smaller than 30. However, the higher frequencies also contain information relevant to the classification as seen in~\cref{fig:imagenet}, where a network trained on the tail achieves over 60\% accuracy.}
    \label{fig:ablation_classification}
\end{figure}

\todo{No longer sure how to bridge to this section if the narrative is condition number -- Rahul}
\subsection{Masked auto-encoders are the new ZCA}

Through our previously results, we have shown the predictive features are present throughout the eigen-spectrum. In the work of \citet{randall_recon} they have inspected how different noise distribution affect the performance, in particular Gaussian white noise has no increase in task performance. Given our results, we know representations learned to be invariant to noised features, still will showcase good task performance given the labels are present throughout the spectrum. One interesting class of noise that has shown difference in task performance is salt and peppers noise, which is effectively the noise distribution used in modern Masked Autoencoders(MAE). These networks mask a certain percentage $\beta$ of the inputs with a given tiling size of $B\times B$. In order to first explore the affect of this strategy on our representations, we looked its influence in the frequency domain Fig. \ref{fig:mae}. We show that these masking strategies for a fixed masking size, actually just nulls out a certain set of frequencies. This nulling strategy is known from the common $sin(x)/x$ function produced from the Fourier transform of a box kernel. Our next question was, why does nulling our frequencies still lead to an increase in task performance. The next answer arose from looking at the eigenvalue spectrum of the original input data and the masked input data distribution. We find that the masking actually influence the condition number of the representation learning problem, by decreasing the condition number it has been shown this makes the optimization problem easier to solve. Given all these connections, we highlight MAE are a novel form of whitening of the input data to learn relevant modes of the data in a optimization-efficient way. 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/mae.pdf}
    \caption{}
    \label{fig:mae}
\end{figure}

Deep networks have been identified to have a frequency bias or a spectral bias when fit on data~\citep{cao2019towards,hacohen2022principal,tancik2020fourier}, i.e., they primarily capture features in the head of the spectrum. However, our results suggests that information is present in the entire spectrum and there is synergistic information in the tail that is unexploited. 
\todo{AB: Can you add a few sentences here on the results?}

% The condition number of the problem comes down because the head comes down.
% in this case, it corresponds to masking.
% we found that masking patches removes certain frequency bands.
% hence, it is doing ``dropout'' in Fourier space. --- if we have masks of different size
% why does the accuracy of linear probing come down... maybe there are objects in images, they have a specific scale.

% if we did randomization over the mask size, then a dropout-like argument can be made to see that we are using all the frequencies equally well. we know that all frequencies are somewhat useful. so how should we force the network to discover the unique information in the different frequencies.

% no matter what mask you select, you are never zeroing out low frequencies. we only zero out the high frequencies. not all of them, in some grating-like pattern


% \subsection{There is more information in the head than the tail, but there are diminishing returns from adding new bands}
% asymmetric in that...from low-frequency to high-freq has a different decay rate than high to low.

\subsection{Redundancy beyond perception tasks: Audition and vocalization discrimination}


Audition, like vision, has a rich literature exploring the links between the properties and patterns of natural stimuli, a nervous system's perception of these stimuli, and the features it learns to arrive at such a perception.\textbf{Citations}. The fields can differ in the vocabulary and methods they use, but they share the same core question: what allows a neural (or, more recently, artificial) system to solve a perceptual task? One successful approach from auditory neuroscience has been probing what changes to stimulus properties yield changes in the perceptual output of observers. Using this approach, the seminal work of Bregman and colleagues \textbf{Citation} was able to show that temporal regularity, that is, the exact way in which sets of frequency evolve over time, played a critical role in perception. Such work has been replicated many times\textbf{Citations}, but the connection between this perceptual result and a set of features a system could learn has not been fully elucidated. Here, we build off of our previous work \textbf{Cite ourselves} and elucidate such a connection. We further demonstrate that, in line with the results presented above, a key auditory task, vocalization discrimination, also has redundancies\textit{some words here that better link to the other paragraphs} just in the temporal domain rather than spatial domain.

Our previous work, in brief, proposed that vocalizations were defined by their particular temporal regularities and demonstrated that learning such regularities allowed a classification network to discriminate between different exemplars of rhesus macaque vocalizations \textbf{Cite ourselves}. Here, we expand on that work in two key ways. First, expanding our data set to include bird song for four different species of bird (American yellow warbler, blue jay, great blue heron, and house finch) \textbf{Cite database} as well as examples from the auditory MNIST \textbf{cite database}. Second, we more thoroughly explore why learning features based temporal regularities worked and link this analysis to our theme of redundancy.  We chose to use slow feature analysis (SFA) \textbf{so many citations} as our algorithm for learning temporal regularities due to its computational tractability and interpretability. The objective of SFA is to find the components of an input signal that have the lowest temporal variance and thus change most slowly over time. Conveniently, this optimization problem can be solved as a generalized eigenvalue problem in a fashion very similar to the more popular principle component analysis. Resulting

In this work we formed 200 pairs of vocalizations for each "animal group": birds, humans, and macaques. We...


% \subsection{Connections between redundancy and masked auto-encoders}

% What are the differences between a masked auto-encoder and a regular auto-encoder?




